Gravitational waveforms in scalar-tensor gravity at 2PN relative order

We compute the gravitational waveform from a binary system in scalar-tensor gravity at 2PN relative order. We restrict our calculation to non-spinning binary systems on quasi-circular orbits and compute the spin-weighted spherical modes of the radiation. The evolution of the phase of the waveform is computed in the time and frequency domains. The emission of dipolar radiation is the lowest-order dissipative process in scalar-tensor gravity. However, stringent constraints set by current astrophysical observations indicate that this effect is subdominant to quadrupolar radiation for most prospective gravitational-wave sources. We compute the waveform for systems whose inspiral is driven by: (a) dipolar radiation (e.g., binary pulsars or spontaneously scalarized systems) and (b) quadrupolar radiation (e.g., typical sources for space-based and ground-based detectors).

==> eqs/splitrhoofv2PNmain.tex <==
\begin{equation}\label{eq:splitrhovmain}
  \rho (v) = \frac{3}{4 \mathcal{S}_-^2 v^7 \zeta \eta} \left[ 1  + v^{2} \rho_{2} + v^{3} \rho_{3} + v^{4} \rho_{4} + \mathcal{O}(5)\right] ,
\end{equation}

